Evorus: A Crowd-powered Conversational Assistant Built to Automate Itself Over Time

Crowd-powered conversational assistants have been shown to be more robust than automated systems, but do so at the cost of higher response latency and monetary costs. A promising direction is to combine the two approaches for high quality, low latency, and low cost solutions. In this paper, we introduce Evorus, a crowd-powered conversational assistant built to automate itself over time by (i) allowing new chatbots to be easily integrated to automate more scenarios, (ii) reusing prior crowd answers, and (iii) learning to automatically approve response candidates. Our 5-month-long deployment with 80 participants and 281 conversations shows that Evorus can automate itself without compromising conversation quality. Crowd-AI architectures have long been proposed as a way to reduce cost and latency for crowd-powered systems; Evorus demonstrates how automation can be introduced successfully in a deployed system. Its architecture allows future researchers to make further innovation on the underlying automated components in the context of a deployed open domain dialog system.

==> conclusion.tex <==
In this paper, we introduced \system, a crowd-powered conversational assistant built to automate over time. \system allows components that automatically propose responses to be integrated, and reduces the need for crowd oversight by learning to help vet potential responses.
%These are integrated into the crowd-powered system using an architecture that allows for increasing automation over time through learning and integration of new automated components over time.
In our deployment, 12.44\% of responses were already automated and 13.81\% of votes were obviated by the automated voting component.
%\jpb{add these numbers if possible}
%Elements of the \system architecture may generally apply to other deployed systems that will be designed to automate themselves over time. 
%\system is designed to automate itself {\em over time}, which we saw some evidence of during the deployment reported on in this paper. 
%We plan to continue to operate it, while improving the automation points, in order to see how it develops over additional time.
Given the complexity of conversational assistance, \system is likely to be crowd-powered in part for some time, but we expect it to continue to increasingly rely on automation. Its architecture provides specific decision points that we believe can be improved upon in future research either separately or as a whole in order to improve performance and automate more of the agent's operation.  


==> conclusion__1_.tex <==
We introduced \system, a crowd-powered system built to automate over time. Informed by two phases of public field deployment and testing with real users, we iteratively designed and refined its flexible framework for open-domain dialog.
We imagine a future where thousands of online service providers can develop their own chatbots, not only to serve their own users in a task-specific context, but also to dynamically integrate their services into \system with the help of the crowd, allowing users to interact freely with thousands of online services via a universal portal.
Supporting this scale offers opportunities for future research.
For example, one direction is to improve the learning framework to support third-party chatbots that also improves overtime, or to better balance between the exploitation and exploration phases (like in a multi-armed bandit problem). \system could also be used to collect valuable fail cases to third party developers for error analysis and improvement of their bots ({\em i.e.}, when a bot was triggered, but its proposed response was rejected by the crowd).

Most automated systems created from crowd work simply use the crowd for data; \system tightly integrates crowds and machine learning, and provides specific points where automated components can be introduced. 
This architecture allows each component to be improved, providing a common research harness on which researchers specializing in different areas may innovate and compete.
The flexibility of the \system framework potentially allows for low cost integration between many online service providers and fluid collaboration between chatbots and human workers to form a single user-facing identity.
Given the complexity of conversational assistance, \system is likely to be crowd-powered in part for some time, but we expect it to continue to increasingly rely on automation.

\section{Acknowledgements}
We thank Walter S. Lasecki and %Lingpeng Kong, and Toni Kaplan.
also the workers who participated in our studies. This project has been funded as part of the Yahoo!/Oath InMind Project at Carnegie Mellon University.

==> discussion_orig.tex <==
%\system is structured in a way that it can automated it
%Malicious chats -> remove message is easier than remove workers
%\system opens up a number of opportunities for future work.

%In this paper, we introduced \system, a crowd-powered conversational assistant built to automate over time. \system allows components that automatically propose responses to be integrated, and reduces the need for crowd oversight by learning to help vet potential responses.
%These are integrated into the crowd-powered system using an architecture that allows for increasing automation over time through learning and integration of new automated components over time.
In our deployment, 12.44\% of responses were automated and 13.81\% of votes were obviated using the baseline automated components we introduced.
%\jpb{add these numbers if possible}
%Elements of the \system architecture may generally apply to other deployed systems that will be designed to automate themselves over time. %
One promising area for improvement is in the automated components used within \system.
For instance, in the experiments we learned that predicting downvotes is more challenging than predicting upvotes.
%Even with a balanced dataset, ``downvote'' class' prediction performance was still far from practical use.
A downvote bot might help messages from misfiring.
%Furthermore,
%Response generation is important, too.
%retrieval-based approach is known to be lack of language understanding capability but only looking for similar context.
%while simple chatbots, such as Filler Bot,
%can contribute to a conversation under \system' framework, significant performance gaps between automated bots and human workers exists.
%better and more chatterbots and task-oriented bots could be included to increase the automation utility in the system.
%Furthermore, for long-term and large-scale deployment, 
%\system is designed to automate itself {\em over time}, which we saw some evidence of during the deployment reported on in this paper. 
%We plan to continue to operate it, while improving the automation points, in order to see how it develops over additional time.
Given the complexity of conversational assistance, \system is likely to be crowd-powered in part for some time, but we expect it to continue to increasingly rely on automation. Its architecture provides specific decision points that we believe can be improved upon in future research either separately or as a whole in order to improve performance and automate more of the agent's operation.  


In this paper, we introduced \system, a crowd-powered system built to automate over time.
%
Informed by two phases of public field deployment and testing with real users, we iteratively designed and refined its flexible framework for open-domain dialog.
%
%that combines artificial intelligent techniques and  crowdsourcing to automatically improves itself over time by interacting with real end-users and learning from the crowds.
%
Most automated systems created from crowd work simply use the crowd for data, but \system tightly integrates the crowd and machine learning, and provides specific points where automated components can be flexibly introduced. 
This architecture allows each component to be improved, providing a common research harness on which researchers specializing in different areas may innovate and compete.
The flexibility of the \system framework potentially allowed for low cost integration between many online service providers and fluid collaboration between chatbots and human workers to form a single user-facing identity. We imagine a future where thousands of online service providers can develop their own chatbots not only to serve their own users in a task-specific context, but also elicit crowdsourcing to dynamically integrate their services into \system, allowing users to interact freely with thousands of online services via a universal portal.


%[10000+ Chatbots]
Our vision of future \system is a system that fuses 10000+ chatbots. To scale up that much, \system may need to be made more robust in various ways; for instance, our current learning framework could better balance between exploitation and exploration phases (like in a multi-armed bandit problem). On the other hand, \system could also collect failed cases to third party bot developers for error analysis ({\em e.g.}, when a bot was triggered correctly but failed to produce quality responses), and the framework would also need to adapt to bot improvements.

%[Evorus talks to Evorus]
%R3 suggested potentials of using crowds to quickly bootstrap the rate of automation.
%We think it's an exciting direction! We could imagine hiring individual workers to interact with Evorus using specific scenarios (e.g., weather), or even have two Evorus' talk to each other. 




%The flexibility of the \system framework potentially allowed for low cost collaboration between many online service providers and integrate many services into a single user facing identity. We imagine a future where thousands of online service provider can develop their own chatbots not only to serve their own users in task specific context, but also elicit crowdsourcing to dynamically integrate their services into the \system framework, allowing users to interact freely with thousands of online services via an universal dialog portal.
%\kenneth{i like the discussion. these 2 paragraph might need merge.}


%our design of 


%Furthermore, since the performance of worker who proposed a message is a critical feature to predict upvtoes, dynamically assigning weights to different workers' votes seems also a promising direction.




%\subsection{After Cold-Start Scenario}
%Prior: Set time window -> it's prob, fine
%Likelihood: Use language model -> how to rank with the original estimates will be a new problem. But this is not entirely new, it's an old problem haha
%When a chatbot has been deployed for a longer time, 


%----------------------- dead kitten -------------------------


\begin{comment}

\paragraph{Bootstraping}

The automated bots included in \system are currently non-task chatterbots. A natural next step is to include task-oriented dialog systems into the mix to allow \system to better handle assistance in domains in which these systems work well. For instance, if the user mentions something about restaurants, a task-oriented restaurant recommender could be included among the candidate responses. If its response is chosen, it might become more likely to provide the next response as well as it moves through its dialog states. A further challenge would be connecting the task-oriented dialog systems together, perhaps using \system as a bridge between them.
Although \system currently contains a relatively small number of automated chatbots, a future goal is to allow multiple chatbots and task-oriented dialog systems to be included at the same time. 
After more than a few are included as potential responders, it will be impossible to show candidate responses generated by all of them to the crowd. At that point, a new machine learning point will likely need to be introduced to select which automated solutions should be polled for candidate responses. Some general purpose systems may also be likely to be included, whereas candidate responses from task-oriented systems may only be included if the context of the conversation so fars suggests they may be relevant.


\end{comment}

==> formative-study.tex <==
\kenneth{Don't think we need this anymore.}
As a formative study, we deployed a quick prototype of \system to twenty real users on Google Hangouts.
This early prototype included all the crowd components ({\em e.g.}, proposing, voting, and the reward system), and it randomly selected one from three external non-task chatbots to participate in conversations.
\system disguised the chatbot as one human worker and crowd workers in Chorus can not tell which responses were proposed by chatbots.
Automatic voting was not implemented in this early prototype.
During 36 conversational sessions, 348 messages were sent by users, 371 crowd messages were accepted, and 41 messages proposed by chatbots were accepted.
We extracted the following key insights, which were later used in developing \system:

\begin{itemize}
    \item In terms of acceptance rate of proposed messages, human workers (71.76\%) outperformed all automated chatbots (24.70\% on average) by a large margin. %are much better thn machines.
    %\item Context is important. Responses extracted from datasets of different context were often unhelpful. In the formative study, the chatbot which was based on transcripts of CNN TV interviews had the lowest acceptance rate. %CNN datset is 10x larger than Chorus dataset, but the acceptance rate is much lower.
    \item Retrieval-based response generation approaches require a careful cleaning on the data it was using. For instance, some responses extracted from TV interviews contained multiple celebrities' names or was too long, which did not fit in the context of personal assistants.
    \item Do not always use only the top answer returned by an retrieval-based response generation model. Known as the ``One True Answer'' problem~\cite{cadwalladr_2016,sullivan_2017} of search engines, some unwanted results might become the only answer from the system if it was always selected and pushed to the user.
    
    %IR-based response generation technologies 
    %IR-based approaches need to be more carefully crafted, e.g., named entities needs to be modified. (Cite Google incident: http://searchengineland.com/googles-one-true-answer-problem-featured-snippets-270549, https://www.theguardian.com/technology/2016/dec/04/google-democracy-truth-internet-search-facebook) Google's ``One True Answer'' problem when featured snippets go bad.
    \item Bots' responses should be visually distinguishable from human workers' responses on worker interface. Multiple workers sent emails to us to report ``malicious workers'' who ``were talking about unrelated things'' and felt the conversation was disrupted.
    
    \item Conversation gap filler such as ``Hi,'' ``Hello,'' or ``What can I help you?'' has a (surprisingly) high acceptance rate, which indicates that simple chatbots can also be useful in \system framework.
\end{itemize}



==> implementation-general.tex <==
\system monitored all ongoing conversations, and periodically called chatbots and vote bots to participate in active conversations.
Both chatbots and vote bots took the entire chat log (including all the accepted, proposed, and expired messages) as input, and generate responses or vote based on the input.
In this study, four chatbots and one vote bot were implemented in \system.
For coordinating with human workers' speed, to each active conversation, \system only proposed no more than one message and sent no more than one vote per minute.
\system randomly selected one chatbot from its chatbot pool each minute, and had the chatbot propose one message to each active conversation whose latest dialogue turn had less than two accepted crowd messages and less than five proposed crowd messages.
If a chatbot decided not to propose any messages, the system proposed ``Hi'' as the default response.
Similarly, \system called the vote bot each minute, and had the vote bot send one (most-confident) vote to each active conversation.
The vote bot can decide not to vote in this turn.
In current \system, the vote bot only voted on the human-proposed messages, but not on the messages proposed by chatbots.
%we required each automatic vote to have at least one extra human upvote to be accepted.
%Vote bots also ignored a message if the same worker proposed the identical content earlier in the conversation but did not get accepted.
%We believe that worker's re-sending is a strong signal of the quality of the message.

%\paragraph{Chorus Data}

%\kenneth{TODO: Write basic stats about Chorus data}
For training a vote bot, we first deployed \system without any automatic bots in October 2016 to collect upvote and downvote data.
%collaborated with the Chorus team~\cite{chorusDeploy} and launched the \textit{downvote} and instant expiration features, which were originally not included in Chorus, in the deployed system in October 2016.
We also obtained the data collected during Chorus' deployment~\cite{chorusDeploy} from May 2016 to March 2017, including all proposed, expired, and accepted messages. 
%with meta data, and the vote records.







%Therefore, both the downvote and upvote 



%It is noteworthy that \textit{downvote} was originally included 
%upvotes and downvotes
%upvote and downvote

==> table/tab-feature.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[t]
\scriptsize
\centering
\begin{tabular}{@{}ll@{}}
\toprule
\textbf{ID} & \textbf{Feature Description} \\ \midrule
\multicolumn{2}{c}{\textbf{Message Level}} \\ \midrule
1 & Vocabulary size of this message \\
2 & String length of this message \\
3 & Worker ID of proposer of this message \\ \midrule
\multicolumn{2}{c}{\textbf{Turn Level}} \\ \midrule
4 & \#Already-accepted crowd message in this turn \\
5 & Duration from the latest user message (sec) \\
6 & \#Already-accepted (and Not-accepted) crowd message of this worker in this turn \\
7 & Word vector of accepted (and non-accepted) crowd messages in this turn \\ \midrule
\multicolumn{2}{c}{\textbf{Conversation Level}} \\ \midrule
8 & \# Accepted (and Not-accepted) messages of this worker in this conversation \\
9 & Duration from the first accepted crowd message in this conversation \\
10 & Duration from the latest crowd message of this worker in this conversation (sec) \\
11 & \# Already-accepted messages in this conversation \\
12 & Message's acceptance rate of this worker in this conversation \\
13 & \# Turns in this conversation \\ \midrule
\multicolumn{2}{c}{\textbf{Word Vector (GloVe)}} \\ \midrule
14 & Average word vector of this message \\
15 & Average word vector of all accepted crowd messages in this turn \\
16 & Average word vector of all not-accepted crowd messages in this turn \\
17 & Average word vector of all the user messages in this turn \\
18 & Difference vectors between any two vectors in \{14, 15, 16, 17\} \\
19 & Element-wise product vectors between any two vectors in \{14, 15, 16, 17\} \\ \bottomrule
\end{tabular}
\caption{Features used in automatic voting. In the feature analysis, the top three features (feature 12, 8, and 6) were all related to the performance of the worker who proposed this message according to history.}
\vspace{-1pc}
\label{tab:feature}
\end{table}
